Graphene-enabled coherent (sub-)terahertz wave detection and thickness determination

Phase-sensitive terahertz (THz) detection enables applications ranging from astronomy to non-destructive testing. However, current THz detectors lack phase sensitivity, unless they are combined with external interferometers, or through photomixing. This implies a large footprint and sensitive dependence on alignment. Here, we demonstrate a graphene-enabled, on-chip, integrated (sub-)THz detector-interferometer with optical cavity and antenna, exhibiting high sensitivity to the phase of incident THz light. We exploit this by determining the thickness of thin films placed in front of the detector-interferometer, obtaining a deep sub-wavelength thickness accuracy of a few micrometer, while we predict that an improved accuracy is within reach. This is relevant for a range of industrial application domains, including automotive, construction, and health. We furthermore achieve a record-high external responsivity - considering bias-free graphene-based (sub-)THz detectors - of 172 mA/W and a noise-equivalent power of 26 pW$~\rm{Hz}^{-1/2}$. This performance is due to enhanced absorption at the resonant cavity mode around 89 GHz, in agreement with multi-physics simulations. These results pave the way to exploiting coherent wave detection in the (sub-)THz regime with utility in spectroscopy, next-generation wireless communication, and beyond.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
     if (!($root_filename eq $_[0]))
     {
         system( "latexmk -cd -pdf \"$_[0]\"" );
     }
 }

